Auto-Formula: Recommend Formulas in Spreadsheets using Contrastive Learning for Table Representations

Spreadsheets are widely recognized as the most popular end-user programming tools, which blend the power of formula-based computation, with an intuitive table-based interface. Today, spreadsheets are used by billions of users to manipulate tables, most of whom are neither database experts nor professional programmers. Despite the success of spreadsheets, authoring complex formulas remains challenging, as non-technical users need to look up and understand non-trivial formula syntax. To address this pain point, we leverage the observation that there is often an abundance of similar-looking spreadsheets in the same organization, which not only have similar data, but also share similar computation logic encoded as formulas. We develop an Auto-Formula system that can accurately predict formulas that users want to author in a target spreadsheet cell, by learning and adapting formulas that already exist in similar spreadsheets, using contrastive-learning techniques inspired by "similar-face recognition" from compute vision. Extensive evaluations on over 2K test formulas extracted from real enterprise spreadsheets show the effectiveness of Auto-Formula over alternatives. Our benchmark data is available at https://github.com/microsoft/Auto-Formula to facilitate future research.

==> latexmkrc <==
# This shows how to use the xr package with latexmk.
# John Collins 2023-03-29
#
# The xr package ("a system for eXternal References") is used by a document
# to make references to sections, equations, etc in other external
# documents. 
# The definitions in this file enable latexmk to apply latexmk to
# automatically update an external document whenever its .tex file changes,
# so that the references in the main document stay up to date.

# Notes:
#    1. This version is defined to put the files from the compilations of
#       the external documents into a defined subdirectory, to segregate
#       potentially many generated files from the main document
#       directories. 
#    2. But for latexmk's custom dependency mechanism to be used, as here,
#       the aux file from compilation of a subdocument must be generated in
#       the same directory as the corresponding source .tex file.  So the
#       .aux file is copied.
#    3. It is assumed that the external documents are to be compiled by
#       pdflatex.  This can be changed, of course, by changing the '-pdf'
#       option given to the invoked latexmk to whatever is needed.
#    4. An ideal implementation would also ensure that recompilation of an
#       external document also happens whenever any of its other source
#       files changes.  But this is not done in the present version, and
#       would probably entail either the use of internal latexmk variables
#       or extra enhancements to latexmk.
#    5. The code uses subroutines copy and fileparse that are loaded by
#       latexmk from the Perl packages File::Copy and File::Basename.
#    6. It also uses some not-yet-documented features of latexmk: an array
#       variable @file_not_found and subroutines popd, pushd, and
#       rdb_add_generated. 


#--------------------
# Configurable choices for compilation of external documents

# Subdirectory for output files from compilation of external documents:
$sub_doc_output = 'output-subdoc';

# Options to supply to latexmk for compilation of external documents:
@sub_doc_options = ();

push @sub_doc_options, '-pdf'; # Use pdflatex for compilation of external documents.
# Replace '-pdf' by '-pdfdvi', 'pdfxe', or 'pdflua' if needed.

#--------------------

# Add a pattern for xr's log-file message about missing files to latexmk's
# list.  Latexmk's variable @file_not_found is not yet documented.
# This line isn't necessary for v. 4.80 or later of latexmk.
push @file_not_found, '^No file\\s*(.+)\s*$';

add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );
sub makeexternaldocument {
    if ( $root_filename ne $_[0] )  {
        my ($base_name, $path) = fileparse( $_[0] );
        pushd $path;
        my $return = system "latexmk",
                            @sub_doc_options,
                            "-aux-directory=$sub_doc_output",
                            "-output-directory=$sub_doc_output",
                            $base_name;
        if ( ($sub_doc_output ne ' ') && ($sub_doc_output ne '.') ) {
               # In this case, .aux file generated by pdflatex isn't in same
               # directory as the .tex file.
               # Therefore:
               # 1. Actual generated aux file must be listed as produced by this
               #    rule, so that latexmk deals with dependencies correctly.
               #    (Problem to overcome: If $sub_dir_output is same as $aux_dir
               #    for the main document, xr may read the .aux file in the
               #    aux_dir rather than the one the cus dep is assumed by latexmk
               #    to produce, which is in the same directory as the .tex source
               #    file for this custom dependency.)
               #    Use not-yet-documented latexmk subroutine rdb_add_generated
               #    to do this:
               # 2. A copy of the .aux file must be in same directory as .tex file
               #    to satisfy latexmk's definition of a custom dependency.
             rdb_add_generated( "$sub_doc_output/$base_name.aux" );
             copy "$sub_doc_output/$base_name.aux", ".";
        }
        popd;
        return $return;
   }
}

==> tables/efficency.tex <==
\begin{table*}
\caption{Average latency on test cases with difference number of reference sheets. "Load sheet" represents the time (seconds) it takes for the user when opening the spreadsheet, while "formula pred." represents the time spent when the user selects a cell to recommend a formula. \sibei{preprocessing / prediction. similar sheet -> online. online -> hist, offline in capition.} }
\label{tab:latency}
\resizebox{1.0 \textwidth}{!}{
\begin{tabular}{|c|cc|cc|cc|cc|}
\hline
                                                                       & \multicolumn{2}{c|}{10}                          & \multicolumn{2}{c|}{100}                         & \multicolumn{2}{c|}{1000}                        & \multicolumn{2}{c|}{10,000}                     \\ \cline{2-9} 
                                                                       & \multicolumn{1}{c|}{Load Sheet} & Formula Pred.  & \multicolumn{1}{c|}{Load Sheet} & Formula Pred.  & \multicolumn{1}{c|}{Load Sheet} & Formula Pred.  & \multicolumn{1}{c|}{Load Sheet} & Formula Pred. \\ \hline
\begin{tabular}[c]{@{}c@{}}Auto-Formula\\ (Sentence-BERT)\end{tabular} & \multicolumn{1}{c|}{57.18}      & 0.265           & \multicolumn{1}{c|}{56.08}      & 1.87           & \multicolumn{1}{c|}{56.43}      & 0.47           & \multicolumn{1}{c|}{46.45}      & 2.11          \\ \hline
\begin{tabular}[c]{@{}c@{}}Auto-Foormula\\ (GloVe)\end{tabular}        & \multicolumn{1}{c|}{0.98}       & 0.11           & \multicolumn{1}{c|}{0.98}       & 0.10           & \multicolumn{1}{c|}{0.98}     & 0.14           & \multicolumn{1}{c|}{0.98}       & 0.45          \\ \hline
Mondrain                                                               & \multicolumn{1}{c|}{2061.72}    & \textless 0.01 & \multicolumn{1}{c|}{9341.82}    & \textless 0.01 & \multicolumn{1}{c|}{34166.19}   & \textless 0.01 & \multicolumn{2}{c|}{TIme Out}                   \\ \hline
\end{tabular}
}
\end{table*}

==> tables/gpt_28_fewshot.tex <==
\begin{table*}
\caption{\add{The F1 scores of GPT's results with few-shot prompts.}}
\begin{tabular}{|c|cccccccccc|}
\hline
                    & \multicolumn{10}{c|}{Few Shot}                                                                                                                                                                                                                                                              \\ \hline
Prompt Engineering  & \multicolumn{2}{c|}{Commen Demos}                          & \multicolumn{2}{c|}{Cheat Demos}                           & \multicolumn{2}{c|}{COT with Cheat Demos}                  & \multicolumn{2}{c|}{RAG Demos}                             & \multicolumn{2}{c|}{COT with RAG Demos} \\ \hline
table Serialization & \multicolumn{1}{c|}{boundary} & \multicolumn{1}{c|}{large} & \multicolumn{1}{c|}{boundary} & \multicolumn{1}{c|}{large} & \multicolumn{1}{c|}{boundary} & \multicolumn{1}{c|}{large} & \multicolumn{1}{c|}{boundary} & \multicolumn{1}{c|}{large} & \multicolumn{1}{c|}{boundary}  & large  \\ \hline
GPT-3.5             & \multicolumn{1}{c|}{0.006}    & \multicolumn{1}{c|}{0}     & \multicolumn{1}{c|}{0.011}    & \multicolumn{1}{c|}{0.039} & \multicolumn{1}{c|}{0.028}    & \multicolumn{1}{c|}{0.033} & \multicolumn{1}{c|}{0.259}    & \multicolumn{1}{c|}{0.246} & \multicolumn{1}{c|}{0.208}     & 0.4    \\ \hline
GPT-4               & \multicolumn{1}{c|}{0.039}    & \multicolumn{1}{c|}{0.028} & \multicolumn{1}{c|}{0.056}    & \multicolumn{1}{c|}{0.039} & \multicolumn{1}{c|}{0.033}    & \multicolumn{1}{c|}{0.044} & \multicolumn{1}{c|}{0.239}    & \multicolumn{1}{c|}{0.161} & \multicolumn{1}{c|}{0.233}     & 0.173  \\ \hline
\end{tabular}

\end{table*}

==> tables/gpt_28_zeroshot.tex <==
\begin{table}[]
\caption{\add{The F1 scores of GPT's results with zero-shot prompts.}}
\begin{tabular}{|c|cccc|}
\hline
                    & \multicolumn{4}{c|}{Zero Shot}                                                                     \\ \hline
Prompt Engineering  & \multicolumn{2}{c|}{-}                                     & \multicolumn{2}{c|}{COT}              \\ \hline
table Serialization & \multicolumn{1}{c|}{boundary} & \multicolumn{1}{c|}{large} & \multicolumn{1}{c|}{boundary} & large \\ \hline
GPT-3.5             & \multicolumn{1}{c|}{0.011}    & \multicolumn{1}{c|}{0}     & \multicolumn{1}{c|}{0}        & 0     \\ \hline
GPT-4               & \multicolumn{1}{c|}{0.044}    & \multicolumn{1}{c|}{0.039} & \multicolumn{1}{c|}{0.033}    & 0.033 \\ \hline
\end{tabular}
\end{table}

==> tables/gpt_description.tex <==
\begin{table*}
\caption{\add{The description of prompt engineering strategies and table boundary detection strategies of GPT.}}
\label{tab:prompts_info}
\resizebox{1.0 \textwidth}{!}{
\begin{tabular}{c|cl|l}
\hline
\multirow{7}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Prompt \\ Engineering\end{tabular}}}       & \multicolumn{1}{c|}{\multirow{2}{*}{Zero-Shot}} & (1) Normal               & Prompts include: task introduction, target table serialization, target cell positions, and output format.                                                                                                                                                                                                                                                                                                                         \\ \cline{3-4} 
                                                                                              & \multicolumn{1}{c|}{}                           & (2) COT                  & Based on the information in normal prompts, we ask GPT to think step by step.                                                                                                                                                                                                                                                                                                                                                     \\ \cline{2-4} 
                                                                                              & \multicolumn{1}{c|}{\multirow{5}{*}{Few-Shot}}  & (3) Common formulas         & \begin{tabular}[c]{@{}l@{}}Based on the information in normal prompts, we add two example demos with a ``SUM'' formula and an \\ ``AVERAGE'' formula.\end{tabular}                                                                                                                                                                                                                                                                \\ \cline{3-4} 
                                                                                              & \multicolumn{1}{c|}{}                           & (4) Common test formulas          & Based on the information in normal prompts, we add some example demos that appear commonly in test cases.                                                                                                                                                                                                                                                                                                                         \\ \cline{3-4} 
                                                                                              & \multicolumn{1}{c|}{}                           & (5) COT with Common test formulas & Based on ``Chead Demos'', we ask GPT to think step by step and explain the steps in example demos.                                                                                                                                                                                                                                                                                                                                \\ \cline{3-4} 
                                                                                              & \multicolumn{1}{c|}{}                           & (6) RAG formulas            & \begin{tabular}[c]{@{}l@{}}Based on the information in normal prompts, we added examples retrieved from the reference set. \\ Our retrieval method have 3 steps:\\ 1. serializing the cells around each formula in the reference set.\\ 2. embedding that sequence using GloVe. \\ 3. Ranking by comparing the similarity of the embedding to the target formula's embedding and select \\    the top 5 as examples.\end{tabular} \\ \cline{3-4} 
                                                                                              & \multicolumn{1}{c|}{}                           & (7) COT with RAG formulas   & Based on ``RAG Demos'', we ask GPT to think step by step and explain the steps in example demos.                                                                                                                                                                                                                                                                                                                                  \\ \hline
\multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Table Boundary \\ Detection\end{tabular}}} & \multicolumn{2}{l|}{(1) boundary}                                          & \begin{tabular}[c]{@{}l@{}}We use a heurstic table boundary detection method to find the table that contain target formula. \\ We move upward from the target cell until we find the first ``string'' cell, which becomes the upper boundary.\\ Then, we extend left/right from this cell until the first ``non-string'' cell is encountered, determing \\ the left/right boundary.\end{tabular}                                  \\ \cline{2-4} 
                                                                                              & \multicolumn{2}{l|}{(2) large}                                             & We use a fix boundary table round the target cell. The size of table is 10*10.                                                                                                                                                                                                                                                                                                                                                    \\ \hline
\end{tabular}
}
\end{table*}

==> tables/train_test_analyze.tex <==
\begin{table}[h]
% \caption{\% of test sheets that have ``similar'' sheets in train set.}
\vspace{-2mm}

\begin{center}
\resizebox{0.4 \columnwidth}{!}{
\begin{tabular}{|c||c|c|c|c||c|}
\hline
    Similarity        & Enron & Cisco & PGE & TI    & Overall-average    \\ \hline
Weak Supervision          & 0     & 0     & 0   & 0.078 & 0.0092 \\ \hline
Jaccard (threshold $>$ 0.3) &  0.0018    &   0   &  0   &   0.012    & 0.011  \\ \hline
\end{tabular}
}
\end{center}
\vspace{-3mm}
\end{table}
